Vortex Formation by Merging and Interference of Multiple Trapped Bose-Einstein Condensates

An apparatus for producing atomic-gas Bose-Einstein condensates (BECs) of 87-Rb atoms is described. The apparatus produces 87-Rb BECs in a dual-chamber vacuum system that incorporates magnetic transport of trapped atoms from the magneto-optical trapping cell to the BEC production cell via the operation of a series of overlapping magnet coils. The design, construction, and operation of the apparatus are described in detail. The apparatus is used to study the creation of quantized vortices in BECs by the merging and interference of multiple trapped condensates. In this experiment, a single harmonic potential well is partitioned into three sections by an optical barrier, enabling the simultaneous formation of three independent, uncorrelated BECs. The BECs may either merge together during their growth, or, for high-energy barriers, the BECs can be merged together by barrier removal after their formation. Either process may instigate vortex formation in the resulting BEC, depending on the initially indeterminate relative phases of the condensates and the merging rate.

==> abstract.tex <==
%An apparatus for producing $^{87}$Rb Bose-Einstein condensates
%(BECs) is described.  The apparatus produces $^{87}$Rb BECs in a
%single-MOT, dual-chamber vacuum system that incorporates magnetic
%transport of trapped atoms from the MOT cell to the science cell via
%a series of overlapping magnet coils.  The design, construction, and
%technical operation of the apparatus are described in detail.
%
An apparatus for producing atomic-gas Bose-Einstein condensates
(BECs) of $^{87}$Rb atoms is described.  The apparatus produces
$^{87}$Rb BECs in a dual-chamber vacuum system that incorporates
magnetic transport of trapped atoms from the magneto-optical
trapping cell to the BEC production cell via the operation of a
series of overlapping magnet coils. The design, construction, and
operation of the apparatus are described in detail.

The apparatus is used to study the creation of quantized vortices in
BECs by the merging and interference of multiple trapped
condensates. In this experiment, a single harmonic potential well is
partitioned into three sections by an optical barrier, enabling the
simultaneous formation of three independent, uncorrelated BECs. The
BECs may either merge together during their growth, or, for
high-energy barriers, the BECs can be merged together by barrier
removal after their formation.  Either process may instigate vortex
formation in the resulting BEC, depending on the initially
indeterminate relative phases of the condensates and the merging
rate.

%Additionally, in a small fraction of experimental runs, single
%vortex cores have been observed to form spontaneously in a symmetric
%trapping potential.



%
%
%This dissertation includes a description of an experiment
%elucidating the relationship between matter-wave interference and
%vortex formation in a Bose-Einstein Condensate (BEC).  In this
%experiment, vortices were formed in a statistical process by the
%merging and interference of multiple trapped BECs. The following
%section is intended to provide some motivation for our interest in
%studying matter-wave interference in BECs, explaining some basic
%concepts along the way.  Section~\ref{section:outline} provides an
%outline of the dissertation.




%This is where the body of your abstract goes, limited to 150 words
%for a thesis, and 350 words for a dissertation or document.  The
%word count limits apply to the regular Abstract in the thesis and
%to the separate Special Abstract.  Use the same text for both; just
%adjust the margins and heading.  The abstract should summarize your
%work.  The UMI booklet listed in the resources section of the U of
%A manual provides some writing tips.  The abstract for a dissertation
%or document may be longer than one page; word count is more important
%than page length in this section.
%
%Submit one copy of the special abstract, and two extra copies of
%your title page, in the box with the final copies of your thesis.


==> acknowledgements.tex <==
First I'd like to thank my advisor, Brian Anderson, for teaching me
the importance of critical thinking, persistence, and working in a
team. Through his mentorship and guidance, Brian has taught me how
to zero in on and think critically about the important parts of a
problem, and, equally importantly, what parts to ignore.  In the
years since I've been working with Brian, what I've learned about
technical problem solving, physical intuition, and working in a team
successfully have been a direct result of his mentorship.

I couldn't have completed this dissertation had it not been for the
contributions of many other students in our group: Chad Weiler,
Tyler Neely, Dave Henry, Elaine Ulrich, Dave Kaz, and Tim McComb.
Chad and I have worked together for many years, and I am continually
amazed by his optimism and positive outlook. Chad's energy seems to
fly in the face of experimental breakdowns or lack of results, when
things get difficult, he is still able to approach everything with a
positive attitude.  Tyler has been a great addition to our research
group, the experiment is in good hands with his meticulous attention
to detail. Until I had worked with Dave Henry, I had never seen so
much enthusiasm in an adult. Dave's persistence, high energy, and
unwillingness to rest until the problem he happens to be working on
is solved will always amaze me.  Elaine built a lot of the early
stages of the experimental apparatus. Dave Kaz provided some of the
funniest and most creative experiences our lab has ever seen, and
Tim McComb built a diode laser in the most impressively efficient
way possible.

It has been a pleasure to interact with several other faculty
members at the University of Arizona. I thank Poul Jessen for
teaching me most of what I know about quantum mechanics, in a
mathematically rigorous way that I really connected with.  I
appreciate Alex Cronin for always asking probing questions, and
being genuinely interested in everything under the sun. Jim Wyant
has been enormously supportive during my time as a graduate student
and I appreciate him as a mentor.

My friends Souma and O have provided camaraderie and companionship
over the many years of working on difficult atomic physics
experiments.

I thank Susan Meyers for her support, friendship, and continued
willingness to go on adventures with me.

Finally, I'd like to thank my parents, my sisters, and all the
members of my extended family.  My parents provided an environment
at home in which creativity and individuality flourished, and always
supported my myriad (and always changing) interests.  I credit that
environment with sparking my initial interest in science, and the
support network of my entire family is what enabled me to finish the
Ph.D.


==> dedication.tex <==
\begin{center}
\emph{To my sisters: Stephanie and Elisabeth}

\end{center}


==> junk/Chap_Background.tex <==
\chapter{Background Information\label{Chap_Background}}

\section{The Concept of Phase in a BEC}
How the overall global phase has no significance.  Description of
the possibility of phase gradients in a BEC.  Discussion of relative
phase between 2 BECs, how this will be relevant to ketterles/our
experiments.
\section{Vortices in Different Superfluid Systems}
Overview of what a superfluid is and how it supports a quantized
vortex.  FIGURE showing a gallery of vortices in different
superfluid systems.
\section{Previous Methods Used to Make Vortices in BEC}
Description of different methods used to made vortices.  FIGURE
showing other vortices
\section{System Check: Making a Vortex Lattice by Rotating an Anisotropic TOP Trap}
Description of how we rotate our TOP trap to make vortices.  FIGURE
showing vortex lattices.  FIGURE showing S-shapes.

%good spinning 8/24/06

\section{Matter-Wave Interference in BEC}
Mainly a description of ketterle's experiments and how different
becs can interfere, displaying interference fringes.  Discussion of
the relative phases of the interfering becs
\section{Spatial Fragmentation of BECs}
Description of what is meant by a fragmented BEC as an alternative
description to our experiment.


==> junk/Chap_Experimental_Long.tex <==
\chapter{Experimental Apparatus\label{Chap_Experimental}}

\section{Introduction}
Construction of a BEC apparatus is govered by two competing, often
contradictory requirements.  Room temperatures atoms need to be
cooled down to temperatures in the nK range and densities as high as
1e12 cm-3.  As there is no one-step method for doing this process
yet, any alkali atom BEC experiment will approach this cooling
process in several steps.  First, room temperature atoms are
collected in a MOT and cooled to uK temperatures.  This prevents the
first requirement: a source of atoms in a region of the vacuum
system that is big enough to allow for large optical beams to
provide the laser cooling.  If you are using dispensers, a side
effect of this requirement will be that the pressure in this region
of the vacuum system will be in the 1e-10 torr range because of the
impurity of the dispensers.

Because laser cooling cannot reach the temperatures needed for BEC,
the atoms must be transferred to a magnetic or optical trap for the
next stage in the cooling process: evaporative cooling.  This brings
us to the second requirement: a region of the vacuum system with
pressure in the 1e-12 torr region that allow for the long lifetimes
necessary to reach BEC.

Most alkali BEC experiments that use dispensers have tackled these
contradictory constraints by building two separate regions into
their vacuum system, a MOT cell and a science cell.  The more
complicated technique of using a Zeeman slower has been described in
detail elsewhere.  We have a dual-chamber, differentially pumped
vacuum system that incorporates two cells, the MOT cell and the
science cell.  We start with a vapor-cell MOT, magnetically transfer
atoms into the science cell 80 cm away, then evaporatively cool the
atoms to the BEC transition in a TOP trap in the science cell.

The organization of this paper is as follows.  Section 1 describes
the physical contruction of a BEC apparatus, with experimental
details on the vacuum system, lasers, magnetic transfer system and
electronics, and TOP trap.  Section 2 describes the timing sequence,
in how all the pieces are put together to form a BEC.  Section 3
describes our imaging and image processing routines.

\section{Physical Construction of a BEC Laboratory}
\subsection{Vacuum System}

Construction of a BEC requires an ultra-high vacuum system capable
of operating at pressures below $1 \cdot 10^{-12}$ torr.  The design
of our differentially pumped vacuum system incorporates two glass
cells, a MOT cell and a BEC cell, separated by 80 cm.  The reason we
have two cells is that these two different regions of the chamber
have vastly different pressure and size requirements. The MOT
requires a large glass cell so that one can use large laser cooling
beams for optimum capture volume, and will operate at a higher
pressure due to the Rb dispensers, which are housed in the MOT cell.
Formation of a BEC requires a very long lifetime in the BEC cell,
which dictates that the pressure in the BEC cell needs to be very
low. Furthermore, the large magnetic field gradients used to trap
the BEC make using a small glass cell desirable.

The MOT cell is a 4 inch x 2 inch x 2 inch rectangular glass cell
that also houses our source of Rb, 4 Rb dispensers.  The MOT is
connected to the main chamber by a 5 mm diameter diaphragm that has
the effect of limiting the vacuum conductance. The MOT is pumped on
by a 20 liter/sec ion pump on the other side of the diaphragm.  The
BEC cell is pumped on by a titanium sublimation pump and a 40
liter/second ion pump. Under normal operations, the two ion gauges,
connected to the two ion pumps, will read $1 \cdot 10^{-10}$ torr.
There is also an ion gauge in the system which can record the vacuum
pressure.

The preparation of vacuum components for use in UHV sitations has
been described in detail elsewhere.  In brief, all stainless steel
components and flanges must be cleaned in deionized water, an
acetone ultrasonic bath, and a methanol ultrasonic bath.  Our vacuum
system then underwent two high-temperature bake-outs.  The first
bake occurred without the glass cells in place and reached a maximum
value of 250 C for 3 days.  After we brought the system back down to
room temperature, the glass cells were attached to the chamber while
performaing a nitrogen purge.  The second high-temperature bake and
degassing of both the Rb dispensers and ti:sub pump filaments then
proceeded.  During this bake, we were careful to not bring the
temperature of the glass above 150 C, and to not have too much of a
temperature gradient between the glass and the connecting flange.
The average temperature of the rest of the system was brought up to
200 C for 3 days.  The dispensers were run at high currents (~5 A)
daily for up to a minute, until they were visibly red-hot.  The
ti:sub filaments were also run daily at high currents.  After 3 days
of baking, the temperature of the system was slowly brough back down
to room temperature, and within 2 days the ion gauge recorded
pressures as low as $1 \cdot 10^{-12}$ torr.

\subsection{Lasers}
The workhorse laser in our experiment is the Coherent MBR-110
ti:sapphire laser, pumped by a Verdi V-10.  The MBR laser is locked
to an atomic transition using a standard saturation spectroscopy
signal.  The layout of the atomic lock is shown in FIGURE.  One
probe beam interacts with the counter-propagating pump to create a
saturated absorption signal, from which is subtracted the pure
Doppler profile generated by a separate non-interacting probe beam.
The saturation signal is modulated by dithering one of the ring
cavity mirrors of the MBR laser, and the obtained subtraction signal
is differentiated using a lock-in amplifier.  The MBR laser is
atomic locked by feeding back an error signal to it's 'external
lock' input, which forces the ring cavity to lock to the external
signal.

The MBR output is sent through a double-pass AOM, a mechanical
shutter, and a single-mode fiber before being split into six
independent MOT beams.  The double-pass AOM allows us to change the
frequency of the cooling beams, and the single-mode fiber is helpful
in improving beam quality and maintaining optical alignment.  A
total of 450 mW is used for the six MOT beams.

Two diode lasers have been constructed using a home-made design. The
diode lasers are Sharp 120 mW diode lasers, which typically have a
free-running wavelength of 784 nm.  An external feedback cavity
employing a holographic grating was built within a Newport Ultima
kinematic mirror mount, and the output was deflected off a mirror in
such a way that grating position did not effect beam steering.  The
schematic of layout, shown in FIGURE, indicates an external grating
diode laser in the ?? configuration, and was adapted from Ref. ??.

The repump laser is locked to an atomic transition using standard
saturated absorption spectroscopy, with a layout similar to FIGURE.
The beam is sent through a single-pass AOM and a shutter, and then
combines with the 4 horizontal beams in the MOT cell.  We use ~30 mW
total power in the repump beam.

A probe diode laser was constructed, using an identical design to
the repump laser.  This laser is atomic locked using a DAVLL lock,
and is used exclusively for far-off resonant phase contrast imaging,
typically with a detuning of ~800 $\Gamma$.

\subsection{Magnetic Transfer System}
A series of 14 pairs of overlapping Anti-Helmholtz coils were
constructed around the vacuum tube to magnetically transfer the
atoms from the MOT cell to the BEC cell.  The magnetically trapped
atoms will be held in a minima of the magnetic field, and by ramping
the coils on in sequence, the minima will move down the tube,
transferring the atoms along with it.  Our design incorporates 3
pairs of coils on at a time, creating a magnetic trap that is
elongated in the longitudinal (transfer) direction.  The coils are
divided into 3 groups, and at any point in time, only one coil pair
from each group will be on. The driving electronics incorporate a
separate switching MOSFET for each individual coil, and 3 pairs of
ramping MOSFETS (one pair for each group) to control the amount of
current.  Thus, 3 analog ramps (to control the amount of current in
each group) and 14 digital lines (to turn on and off each individual
coil) were required in the design.

Most of the transfer coils were 4x8 (axial x radial) turn magnet
coils with an inner diameter of 3.25 cm, constructed using 32 AWG
magnet wire. The coils have an inductance of 100 $\mu$H and a
resistance of 110 m$\Omega$.  The coils are mounted on copper plates
above and below the transfer tube.  Both the coils and the MOSFETS
are situated on on water-cooled copper plates to reduce the amount
of heating during the transfer process.

Conditions for adiabatic transfer from the MOT cell to the science
cell require that the axial and radial magnetic field gradients not
change appreciably during the transfer process, ideally they would
stay the same as the atoms progress down the transfer tube.  Another
condition is the the velocity of the B=0 point (and thus the atoms)
would not move faster than atomic motion due to oscillations within
the confining potential.

A 3-dimensional simulation was performed to determine the current
ramps necessary to produce the desired magnetic field gradients. The
simulation determined what currents were necessary to provide the
required field gradients and a B=0 point at a desired location. The
required current ramps and resultant magnetic field gradients are
shown in FIGURE. Transfer of magnetically trapped atoms from the MOT
cell to the BEC cell (80 cm) takes ~4 seconds, and is not very
dependent on transfer velocity, initial acceleration, or final
deceleration.

Two power MOSFETS are required to turn on each coil, a switching
MOSFET used to turn the individual coils on/off, and a ramping
MOSFET which effectively acts like a variable resistor, governing
the amount of current flow in that coil group. There is a flyback
power diode placed in parallel with each coil pair to dissipate
current spikes due to inductive kicks. The transfer coils operate on
a linearized feedback loop shown in FIGURE. The transfer circuit
monitors how much current is flowing through an individual coils via
a Hall Probe and applies this feedback signal to the gate of the
controlling MOSFET. Without this feedback loop, when a MOSFET gets
hot and its resistance changes, the current through the coil would
also change, but the feedback loop prevents this thermal runaway by
always monitoring the amount of current flow and applied the proper
voltage to the gate of the ramping MOSFET.

\subsection{TOP Trap}
After the magnetic transfer into the BEC cell, the atoms are held in
a quadrupole trap by the final transfer coil pair, pair 14. The
atoms are then transferred into the TOP trap.  The TOP trap coils
are concentric with the final transfer coils and held on the same
mount, but lie closer to the BEC cell. The TOP trap is an axially
symmetric trap created by the addition of the two TOP trap coils and
the AC coils, two pairs of Helmholtz coils that provide a rotating
radial bias field. The two rf coils are each made up of one single
loop of magnet wire, above and below the BEC cell, wired in
Helmholtz configuration.  Because of the long evaporation times, the
TOP trap coils heat up to a temperature that is hotter than any
other coils used in the transfer process.  This could pose a problem
with overheating of the BEC cell, since the coils lie only a few mm
from the glass cell. However, forced air cooling created by a
directed fan alleviates the overheating.

The desired rf frequencies are created with an Agilent E4400B rf
synthesizer and amplified using an OPHIR rf amplifier, then sent to
the rf coil.  The AC field is generated by applying a 2 kHz sine
wave into the input of a Crown XLS402 power audio amplifier, then
sent to the AC coils. A function generator is AM-modulated to change
the amplitude of the AC coils' driving field.

\subsection{Computer Timing System}
A complex timing program, using the software packages LabVIEW and
Matlab, was written to control all aspects of the experiment.  The
program is capable of reading in analog inputs and controlling the
experiment using analog and digital outputs.  The program creates a
BEC, performs an experiment, and then records the output by
triggering an image acquisition on a CCD camera.  A separate
computer controls the CCD camera and is used for image acquisition
and analysis.

The workhorse computer board in our experiment is the Viewpoint
DIO-128 digital output board, which has 4 ports of 16 digital output
lines each. This board is used to turn on and off various devices in
the experiment, such as shutters, AOMs, magnets, etc.

Each digital line on the DIO-128 must be carefully isolated so as to
avoid ground loops.  A potential problem occurs when an
electromagnetically reflected signal is sent back to the computer,
which can kill a board. To prevent this, isolation of the computer
ground from the lab ground is necessary.  Each digital line is first
sent through an Agilent HPCL-220 opto-isolator, which isolates the
input and output grounds optically.  Then each signal is sent
through a TI SN74128 line driver that provides the digital line with
additional current output.  This is done for all of the digital
lines directly after the DIO-128 ribbon cable, before they connect
to lab devices.

A 16-bit Digital-to-Analog Converter (DAC), Analog Devices AD7846JN,
is used to generate a high-resolution analog signal from 16 digital
lines on the DIO-128. This method of analog signal generation has
the benefit of ensuring that the digitally derived analog signal is
exactly synchronized with all the digital lines already being used,
and allows us to generate analog and digital signals using only
oneboard.  The DAC signal is used simultaneoulsy to control the
varying MOT current at the first stages of the transfer sequence and
the TOP trap current during the evaporation sequence.

A NI PCI-6023E board is using for analog input.  One channel on this
board reads the voltage level on a photodiode monitoring the MOT
fluorescence and proceeds with the rest of the timing sequence only
when a certain voltage has been reached.  This ensures that we start
out with the same number of atoms in the MOT every run of the
experiment.

A NI PCI-6713 analog output board is used to control the devices
that need to vary continuously in the MOT loading portion of the
sequence, such as the cooling laser intensity and detuning, and the
repump laser intensity.  The analog output board is not fully
isolated from lab ground like the DIO-128 board is, however, a
differential amplifier is placed along each line to separate
computer ground from lab ground by 240 k$\Omega$.

\section{Putting it all Together: Creating a BEC}
\subsection{Complete Timing Sequence}
The complete timing sequence used to create a BEC is shown in FIGURE
and will be described in five steps, creating a MOT, the CMOT phase,
magnetic transfer to the BEC cell, transfer to the TOP trap, and
evaporative cooling.
\subsection{MOT}
The MOT uses 6 independent counter-propagating cooling beams, with a
total of 450 mW in the 6 beams.  We have used diverging beams as the
MOT beams in order to increase the capture volume in the MOT cell
without needing to use 2 inch diameter optics. The diverging beams
also make the MOT less susceptible to optical misalignment and
standing-wave patterns caused by counter-propagating collimated
beams. The diverging beams are creating by sending 2 cm diameter
beams into an f=100 mm, 1 inch diameter lens placed 400 mm from the
center of the MOT cell. We estimate that the beams have a diameter
of 10 cm at the location of the MOT, resulting in a total intensity
of 2.9 mW/cm$^{2}$ = 1.8 $I_{sat}$. The MOT beams are tuned 4
$\Gamma$ below the $F=2 \rightarrow F'=3$ transition.

The repump beam is split into the 4 horizontal arms of the MOT, and
travels along the same path as the cooling beams, resulting in 4
diverging beams with a diameter of 10 cm at the MOT location.  We
use a total of 30 mW in the repump beam, resulting in a total
intensity at the MOT of 0.19 mW/cm$^{2}$ = 0.12 $I_{sat}$.

The magnetic field gradient produced by the MOT coils is 8 G/cm
during the MOT loading phase.

A photodiode placed near the MOT cell records fluorescence from the
MOT, and based on the amount of fluorescence and the scattering rate
caused by the cooling beams, we can calculate the number of atoms in
the MOT.  The total power emitted during a fully-loaded MOT in all
directions is equal to the number of atoms in the MOT times the
probability of photon emission times the energy per photon, divided
by the natual lifetime of the transition.

$Power_{emitted} = (N_{atoms}) \cdot P_{emission} \cdot E_{photon} /
lifetime$

$P = N \cdot (1/2 \cdot I/I_{sat} / (1 + I/I_{sat} + 4 \cdot
(\Delta/\Gamma)^2 \cdot h \nu_{Rb} / \tau_{nat}$

Knowing that our photodiode only collects a small fraction of the
total solid angle of fluorescent light, and knowing the intensity in
the cooling beams, we calculate the number of atoms in the MOT to be
$3 \cdot 10^9$ atoms.

Our MOT has a $(1-1/e)$ filling time of 15 seconds with the Rb
dispensers running at 3.4 A, and fills to $3 \cdot 10^9$ atoms. The
temperature of the atoms in the MOT is ?? uK, and the cloud size is
1 cm diameter, easily visible with the human eye.

\subsection{CMOT}
The compressed MOT (CMOT) phase of our experiment spatially
compresses the MOT and causes a momentary increase in density, which
aids in the loading of ultracold atoms into a magnetic trap. The
dominant player in the CMOT phase is the repump intensity. By
turning the repump intensity down for a short period of time, we
allow a sizeable population of atoms to build up in the F=1 state
and stay out of the cooling beams.  The CMOT phase is 40 ms long and
consists of ramping the cooling beam detuning from -4 $\Gamma$ to
-10 $\Gamma$ (the intensity will also decrease by a factor of ??),
ramping the magnetic field gradient from 8 G/cm to 2 G/cm, and
switching the repump power from 30 mW (full power) to ?? for the
duration of the CMOT phase. The temperature of the atoms after the
CMOT is ??, and the cloud is now ?? in diameter.
\subsection{Optical Pumping}
After the CMOT phase, the cooling beams (still at the CMOT detuning)
and magnetic field (still at 2 G/cm) stay on for an additional 2 ms
longer than the repump beams, forcing all the atoms to populate F=1.
Having the cooling beams and magnetic field on at the same time
prevents us from populating any atoms in the F=2 state of our
magnetic trap.  Then, the cooling beams are turned off and the
magnetic field gradient is switched on to 50 G/cm.  This traps atoms
in the F=1, m$_f$ = -1 state.
\subsection{Magnetic Transfer}
The magnetic field gradient in the MOT coils is ramped up from 50
G/cm to 170 G/cm in 100 ms, and then the transfer sequence begins.
Transfer coils 1, 2, 3, etc. will turn on in sequence, with 3 coils
normally on at a time.  The transfer process, over a distance of 80
cm, takes 4 sec.  There is a 5 mm diameter circular diaphragm
between the MOT cell and the transfer tube, which has the effect of
limiting vacuum conductance from/into the MOT cell.  However, this
diaphragm was not perfectly aligned with the transfer coils B=0
point, and push coils must be used to shift the B=0 point during
passage through the diaphragm.  An axial current of 19 A and a
transverse current of 1.7 A through our push coils are required to
shift the fields by the necessary amount.  Starting with $3 \cdot
10^9$ atoms in the MOT, we transfer about $3 \cdot 10^8$ atoms into
the quadrupole trap in the BEC cell.
\subsection{Transfer to TOP Trap}
Immediately after transferring the atoms into the science cell, we
apply a short pulse of light near-resonant with the F=2,F'=3
transition to drive away any wayward atoms that are still
magnetically trapped in the F=2 state in the science cell due to
imperfect optical pumping.  This pulse, referred to as the 'kill
pulse', if 5 ms long and is not very dependent on laser intensity or
detuning. It will increase the number of atoms in the final BEC
slightly by removing any F=2 atoms, which only provide collisions
that are deleterious to the evaporative cooling process.

At the end of the transfer process, the atoms are trapped in a
quadrupole field created by the final transfer coil pair, coil pair
14, at an axial gradient of 180 G/cm. The atoms are then transferred
into a quadrupole field created by the TOP trap coils, concentric
with coil pair 14. This is done by ramping the current in coil pair
14 down to zero while ramping up the TOP trap coils from zero to an
eventual field gradient of 180 G/cm over 100 sec. The atoms are then
transferred into the TOP trap by switching the axial field gradient
from 180 G/cm to 300 G/cm and simultaneously turning on the rotating
radial bias field to 41 G, at 2 kHz. We have measured magnetic trap
lifetimes in the BEC cell as long as 8 minutes in the 180 G/cm
quadrupole field, and were limited in the TOP trap lifetime
measurement by heating of the TOP coils. We start out with 1e8 atoms
in the TOP trap at a temperature of ?? K and size is ?? mm.
\subsection{Evaporative Cooling}
Evaporative cooling is accomplished by decreasing the radial bias
field, thus bringing the rotating B=0 point (the circle of death)
closer to the origin, while simultaneously decreasing the rf
frequency. The rf field is created by a pair coils in Helmholtz
configuration that send a time-varying magnetic field oscillating at
an rf frequency onto the cloud of atoms. Because the atoms are in a
spatially varying magnetic field, the cloud experiences spatially
varying Zeeman shifts, and the rf frequency will be tuned to be in
resonance with only the periphery of the cloud, ejecting atoms from
the trap by driving them into untrappable magnetic sublevels.

The evaporation process occurs in two phases.  Phase I is in the 300
G/cm TOP trap and cools the atoms to a point just above the BEC
critical temperature.  Then, the axial field gradient is reduced,
placing the atoms in a weakly confining potential that allows us to
generate spatially larger BECs. The phase II evaporation, which
cools the atoms through the BEC critical temperature, occurs in this
weakly confining TOP trap.

Phase I evaporation occurs over 70 seconds.  In the first 60 seconds
the rf frequency ramps from 70 MHz to 7 MHz, and the rotating bias
field changes ramps from 41 G to 5 G.  During this phase the rf
frequency changes along with the bias field such that the rf
frequency is always ejecting atoms that lie right at the circle of
death.  All ramps are done with a decaying exponential ramp with a
time constant approximately equal to the time of the ramp.

For the rest of the sequence the bias field is left at 5 G and all
further evaporation is done solely with the rf frequency. In the
next 10 seconds the rf frequency is brought from 7 MHz to 4.5 MHz,
this corresponds to a point just above the critical temperature.

Then the atoms are moved to the gravity-sagged TOP trap by reducing
the axial field gradient from 300 G/cm to 55 G/cm over 2 sec, using
a nonlinear current ramp that approximates a linear shift in B=0
point over the sag time.  The atoms sag 0.6 mm in this time due to
the larger role played by the gravitational potential in the weak
trap compared to the tight trap. During the sag process the rf
frequency is brought up to a higher value of 5 MHz to prevent
additional evaporative cooling.

Phase II evaporation occurs in the gravity-sagged TOP trap with an
axial field gradient of 55 G/cm and radial bias field of 5 G.
Because the atoms no longer lie at the center of the TOP trap coils,
the Zeeman shifts are different at the top and bottom of the cloud,
and evaporation only occurs at the bottom (the south pole) of the
atomic cloud. This 1-D evaporation is significantly less efficient
than the 2-D (around the equator) evaporation afforded by
evaporation in a tight TOP trap, and evaporation times need to be
correspondingly longer.  Phase II evaporation brings the rf
frequency from  5 MHz to 4.7 MHz over 20 seconds, and a pure BEC is
observed. The phase II evaporation time can be decreased to as short
as 5 seconds, but there will be a reduction in the number of atoms
in the BEC.

The propagation of rf frequencies through an antenna has other
serious consequences in our lab, such as driving lasers out of lock
or making temperature controllers finicky.  For frequencies in the
range of 11 to 16 MHz, we need to decrease the rf power from its
nominal value of -5 dBm to -15 dBm, and between 16 and 23 MHz we
decrease the power to -23 dBm.  The rf coil also has different
responses to different frequencies, and we boost the power in the
ranges from 31 to 36 MHz as well as 43 to 52 MHz up to -3 dBm.
(!!CHECK ATTENUATOR!!)

We have measured the trap frequency in the tight 300 G/cm, 5 G TOP
trap to be $\omega = 2\pi \cdot$ 39.8 Hz, and the trap frequency in
the gravity-sagged 55 G/cm, 5 G trap to be $\omega = 2\pi \cdot$ 7.3
Hz.

After rf cooling the atoms through the BEC transition temperature in
the gravity-sagged trap, we end up with a pure BEC with an axial
Thomas-Fermi radius of a$_z$ = 40 $\mu$m and a radial radius of
a$_z$ = 28 $\mu$m, with $2 \cdot 10^6$ atoms in the BEC.

\section{Imaging}
\subsection{Overview, physical description of imaging system}
We have set up a vertical and horizontal axes, both capable of
either absorption or phase-contrast imaging, in order to image the
cloud from 2 directions.  Because of the geometry of the BEC cell,
the vertical imaging passes through two 1 mm thick glass surfaces
separated by 10 mm, producing some fringes on the beam that are not
present on the horizontal axis.

We typically use phase-constrast images taken of the BEC in the
gravity-sagged trap or immediately after release from the trap in
order to characterize the number, size, and temperature of the
cloud.  In expansion images, the size of the cloud has increased by
enough that absorption imaging is necessary.

We create a condensate in the F=1, $m_F=-1$ state, but the
near-resonant light used for absorption imaging drives the F=2, F'=3
transition, so we need a way to optically pump the atoms from F=1
into F=2. We do this by a short pulse of light, referred to as the
repump flash, in resonsance with the F=1,F'=2 transition.  The
repump flash occurs in free space, using a pulse of 10 $\mu$s
duration with ?? mW of laser power.  We have found that longer or
more intense repump flash pulses significantly degrade the quality
of absorption images, resulting in clouds that have expanded by 2 or
3 times in size.  For phase-contrast images, we use light that is
far-off resonant with the F=1,F'=2 transition, so optical pumping is
not necessary.


\subsection{Layout of imaging systems}
A schematic of the horizontal and vertical imaging systems are shown
in FIGURE.  Both imaging systems were designed using the optical
design software ZEMAX, which allowed us to design
diffraction-limited optical systems.  The horizontal system used 4
achromats (2 groups of 2 paired achromats) and passes the image
through an intermediate image plane.  The vertical system only uses
2 achromats total has a collimated intermediate image space rather
than an intermediate image plane.  In both cases, a phase dot is
slipped into or out of the focus of the probe laser beam to shift
the phase of the laser light by $\pi$/2 relative to the BEC image
light, which is much larger than the 200 $\mu$n diamter phase dot.
This allowed us to easily switch between phase-contrast and
absorption imaging by simply moving a phase dot.  Both imaging
systems have an optical magnification of 5.6, which was measured
experimentally by calibrating the distance a cloud of atoms fell
ballistically due to gravity.

\subsection{Image processing and image analysis}
Images were taken by triggering a Princeton Instruments PIXIS CCD
camera.  Three frames are taken for each data run, a shadow,
background, and dark frame.  The shadow frame consists of the probe
laser beam passing through the BEC, the background consists of the
same probe laser beam shining directly onto the CCD camera, and the
dark frame consists of an image exposure with no light present. The
dark frame is subtracted from the shadow and background frames to
get rid of the effects of room lights, stray light, and bad pixels.

We have constructed a comprehensize image processing program in
matlab that will process images of thermal, bimodal, or bec clouds
and provide relevant parameters.  The program is adaptable for
either absorption or phase-contrast imaging, and is variable for use
with either the horizontal or vertical imaging systems.  The basic
algorithm is as follows: an array labeled 'optical depth' is
contructed, based on either the absorption or phase-contrast imaging
scenarios, corrections for detuning or saturation effects are
applied to the optical depth array, the image gets smoothed and/or
filtered, then that image is fit to either a Gaussian distribution,
Thomas-Fermi distrubtion, or a combination of the two to extract
relevant parameters.

For absorption imaging the raw optical depth is generated as $OD =
-log(shadow/back)$.  We have measured experimentally that the
maximum OD we can measure with our system is 3.3, and we apply a
nonlinear correction to the OD based on this maximum measurable OD.
Using $\alpha = e^{-(OD_{max})}$, we can define $OD_{corrected} =
-log((shadow - \alpha \cdot back) / (back - \alpha \cdot back))$.







% more sections that need to be written

% how we calculate Nbec, image processing etc
% more specifics on spectroscopy for laser locks
% expansion coil
% more on diode laser construction

% shoot for 50 pages on experimental section


==> junk/chapter_1.tex <==
\chapter{Introduction\label{Chap_Introduction}}


\section{Introduction}

I wouldn't actually name any of my chapter files chapter1.tex,
chapter2.tex, etc.  You might decide to swap them around at some
point, and then things can get messy, especially if you've labeled
things inside those files with labels like ``chap1.''  Computers
are good at counting things, let \LaTeX\ do that for you.  Be general
with your naming scheme, you can always rearrange things by altering
their order in the main dissertation.tex file.


\section{Math Example\label{math}}

This is a real short example of using the equation environment.

\begin{equation}
    y = mx + b
\end{equation}

There is an awful lot that the equation environment and math mode
can do for you.


\section{How to cite your references\label{ref_citation}}

Here is an example of references using the natbib package and
`uabibnat.bst' file.  You can reference in a number of ways.  The
ones that are most useful are parenthetical \citep{article,articletwo}
or inline, as in \citet{articletwo} said this or that.  You can
also include information within the citation \citep[e.g.][doesn't
have any page numbers]{2003jgr}.  You don't even need to have the
reference in your text to be included.  \nocite{2004LPI}

For other ways of referencing, you can read more about the natbib
package by reading its documentation.  You should be able to find
the DVI file on your system where natbib was installed.  On my
system it's at /usr/local/share/texmf/doc/latex/natbib/natbib.dvi.


\section{Graphics\label{graphics}}

On the next page is a figure inclusion using the `graphicx' package.
This puts figures on their own page by themselves.  They don't need
to be on separate pages, there is no requirement that they be on
separate pages.  If you want to put a figure on a page with text,
don't include the \emph{p!} option in square brackets at the begin
figure command (as I have commented out below).

Also note that the \verb=\caption= command has an optional
square-bracketed argument and a curly-bracketed argument.  Whatever
you put in square brackets will be used as the short caption, and
will go into the List of Figures.  The stuff in the curly brackets
will be placed on the page under your figure.

% \begin{figure}
\begin{figure}[p!]
\begin{center}
\includegraphics{figure.eps}
\caption[Short figure caption for LOF]{Sample figure caption (to appear below
the actual figure). \label{samplefig}}
\end{center}
\end{figure}


==> junk/chapter_2.tex <==
\chapter{Sample Second Chapter\label{chap2}}

\section{Remembering to use non-breaking spaces}

The tilde character can be used to mark a non-breaking space.  \LaTeX\
does a great job of lining words up, putting in line breaks where
appropriate, and making the text flow properly.  However, there are
some cases where you really don't want \LaTeX\ to toss in a carriage
return.  The places that spring to mind are between numbers and
their units, and between Figure and Table references and their
values.  So for example, you don't want something like this in your
document:

\begin{quote}
	Blah blah blah blah blah blah blah blah blah is 10\\
	m from foo to bar.
\end{quote}

So always use the tilde when you use numbers with units, like
9.8~m~s$^{-2}$, and with Figure and Table references, like
Figure~\ref{samplefig} and Table~\ref{sampletable}.  This way \LaTeX\
will never put a line break between those elements.


\section{Tables\label{tables}}

On the next page is a sample table, placed on the page by itself.
Again, this table is pretty small, so it could probably just be
placed on a page with text.  Messing with tables can be quite
grueling, so find yourself a good book.  Sometimes tables can be
wider than they are tall, and you may need to rotate the table by
$90^{\circ}$ to make it fit better on a page by itself.  To do that
you can use the lscape package.  To use it, you need to do two
things, uncomment the usepackage statement in the main dissertation
file, and wrap the table commands in a begin and end landscape
command (like I have commented out in this file), and that table
will be properly rotated.  Go ahead, try it out.

% \begin{landscape}
\begin{table}[p!]
\begin{center}
\caption[Short table caption for LOT]{Sample table caption (to appear with the actual table). \label{sampletable}}
\vspace{0.3in}
\begin{tabular}{ccc}
\hline 
\hline
Col A & Col B & Col C \\
\hline
1 & 2 & 3 \\
4 & 5 & 6\\
\hline
\end{tabular}
\end{center}
\end{table}
% \end{landscape}

Note that the \verb=\caption= command can have a short and a long version
inside a table environment, just like inside a figure environment (see \ref{graphics}).

